Bandit on the Hunt: Dynamic Crawling for Cyber Threat Intelligence

Public information contains valuable Cyber Threat Intelligence (CTI) that is used to prevent future attacks. While standards exist for sharing this information, much appears in non-standardized news articles or blogs. Monitoring online sources for threats is time-consuming and source selection is uncertain. Current research focuses on extracting Indicators of Compromise from known sources, rarely addressing new source identification. This paper proposes a CTI-focused crawler using multi-armed bandit (MAB) and various crawling strategies. It employs SBERT to identify relevant documents while dynamically adapting its crawling path. Our system ThreatCrawl achieves a harvest rate exceeding 25% and expands its seed by over 300% while maintaining topical focus. Additionally, the crawler identifies previously unknown but highly relevant overview pages, datasets, and domains.

==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}
This section gives specific details about the implementation of each concept mentioned in \cref{sec:theoretical_concept}.

\subsection{Used Libraries}
As mentioned in \cref{subsec:architecture}, a new crawler called \threatcrawl{} had to be developed.
To make \threatcrawl{} as simple and lightweight as possible, native Python was used primarily.
The following libraries/modules are the only ones used in addition to the built-in ones:
\begin{itemize}
    \item Beautiful Soup\footnote{\url{https://www.crummy.com/software/BeautifulSoup/}}: Library for parsing, traversing, and manipulating \ac{html} content and documents.
    \item Protego\footnote{\url{https://github.com/scrapy/protego}}: Library for parsing robots.txt files
    \item NumPy\footnote{\url{https://numpy.org/}}: Scientific computing library
    \item PyTorch\footnote{\url{https://pytorch.org/}}: \ac{ml} framework
    \item Transformers\footnote{\url{https://pypi.org/project/transformers/}}: Library for loading and manipulating tokenizers and \ac{ml} models
    \item Trafilatura\footnote{\url{https://trafilatura.readthedocs.io/en/latest/}}: Library for discovering and extracting web content
\end{itemize}

To extract the main content of a web page, \threatcrawl{} uses Trafilatura~\cite{barbaresi_trafilatura_2021}, which provides a simple function that extracts the main content of a \ac{html} document and returns it as parsed and plain text.

A domain blacklist is essential for blocking common domains such as Youtube or Facebook.
Sites like these are widely used, but are of no use when searching for \ac{cti} relevant information, especially when focusing on text documents.
Worse, since many of them hide their content behind logins, they cannot even be considered part of the Clear Web.
Unfortunately, there is no realistic list of all websites that are not part of the Clear Web. %Beide sätze hintereinander enden fast identisch
Therefore, the top 100 most used sites were used as a starting point to filter out sites that typically do not provide content relevant to this work.

Since no suitable dataset was available, a new one had to be created.
This was done by selecting several blogs and websites that contained articles with \ac{cti}-relevant information as defined in \cref{subsec:what_ist_relevant}.
This resulted in a data set of 259 \acp{url}.
Of these 259 \acp{url}, 153 were labeled \emph{relevant} and 106 were labeled \emph{not relevant}.
For a more precise classification, the label \emph{relevant} was divided into sub-labels.
The final dataset therefore consists of the following documents per label:
\begin{itemize}
    \item Relevant: 153
    \begin{itemize}
        \item \ttplabel: 55
        \item \infolabel: 24
        \item \malwarelabel: 36
        \item \vulnlabel: 38
    \end{itemize}
    \item Not Relevant: 106
\end{itemize}

It is important to note that the sub-labels often overlap.
For example, articles describing \acp{ttp} also contain information about the malware used and the vulnerabilities it targets.
This can also be seen in the analysis of the most important sentences per label~\see{subsec:eval_classifier}.
In \cref{fig:dataset} you can see the number of extracted sentences per label.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/dataset.png}
    \caption{Sentences per label in dataset}
    \label{fig:dataset}
\end{figure}

\subsection{Contextualized Embeddings}
To create the contextualized embeddings, a pre-trained \ac{bert} model called CySecBERT~\cite{bayer_cysecbert_2022} was used.
CySecBERT is a fine-tuned version of the \emph{bert-base-uncased} model and was trained on 528M tokens collected from content in the IT security environment.
The resulting model has 12 hidden layers with 768 hidden units in each layer.

Before embedding a sentence, it must be preprocessed by tokenizing it. This involves adding the start token and the delimiter token at the end: 
\[\mathrm{Input}(sentence)=[\mathrm{CLS}]\;\mathrm{Tokenize}(sentence)\;\mathrm{[SEP]}\]

Since the input layer can only handle a maximum of 512 tokens, any token above this limit must be removed.
\cite{devlin_bert_2018} notes that concatenating the last four hidden layers achieves high scores even without fine-tuning the model.
Using the result of the last four layers, a contextualized embedding is created for each token in the sentence.
Since each layer contains 768 hidden units, each embedding has a length of 4 * 768 = 3027.
These token vectors can then be summed to form sentence vectors, which can then be summed to form a single document vector. %"can then be" 2x hintereinander stört den Lesefluss ein bisschen

\paragraph{Adaptive number of sentences}
To calculate the number of sentences, sentence gradients were calculated for all relevant documents in the dataset~\see{fig:sentence_gradients}.
A value of 0.02 was chosen as the minimum that must be reached before no more significant value is gained by considering more sentences.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/sentence_gradients.png}
    \caption{The Sentence Gradients}
    \label{fig:sentence_gradients}
\end{figure}

\paragraph{Choosing the right seed}
To maintain reproducibility, a fixed seed was used.
The seed consists of 51 \acp{url} with a wide variety between sites that typically host \ac{cti} relevant content and sites that do not.
Some of the domains in the seed are also found in the dataset, and some are completely new.
